Handwriting-Based Gender Classification Using End-to-End Deep Neural Networks

Handwriting-based gender classification is a well-researched problem that has been approached mainly by traditional machine learning techniques. In this paper, we propose a novel deep learning-based approach for this task. Specifically, we present a convolutional neural network (CNN), which performs automatic feature extraction from a given handwritten image, followed by classification of the writer's gender. Also, we introduce a new dataset of labeled handwritten samples, in Hebrew and English, of 405 participants. Comparing the gender classification accuracy on this dataset against human examiners, our results show that the proposed deep learning-based approach is substantially more accurate than that of humans.

==> images_sections/full_form_example_imgs.tex <==
\begin{figure}
\centering  
         \begin{subfigure}[t]{0.4\textwidth}
                \centering
                \fbox{\includegraphics[width=\textwidth]{images/form_11e_full.png}}
                \caption{}
                \label{fig:engForm}
        \end{subfigure}
        ~ \hspace{2cm}
        \begin{subfigure}[t]{0.4\textwidth}
                \centering 
                \fbox{\includegraphics[width=\textwidth]{images/form_11h_full.png}}
                \caption{}
                \label{fig:hebForm}
        \end{subfigure}
        
        \caption{Examples of: (a) English and (b) Hebrew handwriting forms from the HEBIU dataset.}
        \label{fig:full_forms_example}
%\includegraphics[width=60mm,height=60mm]{a.jpg}
\end{figure}


==> images_sections/hw_classification_and_misclassification_imgs.tex <==
\begin{figure}
\centering
         \begin{subfigure}[t]{0.4\textwidth}
                \centering
                \fbox{\includegraphics[height=2.5cm, width=5cm]{images/form_305_male_as_male.png}}
                \caption{}
                \label{fig:engSection}
        \end{subfigure}
        ~ \hspace{1cm}
        \vspace{0.2cm}
        \begin{subfigure}[t]{0.4\textwidth}
                \centering
                \fbox{\includegraphics[height=2.5cm, width=5cm]{images/form_281_female_as_female.png}}
                \caption{}
                \label{fig:hebSection}
        \end{subfigure}
        
         \begin{subfigure}[t]{0.4\textwidth}
                \centering
                \fbox{\includegraphics[height=2.5cm, width=5cm]{images/form_150_male_as_female.png}}
                \caption{}
                \label{fig:hebSection}
        \end{subfigure}
        ~ \hspace{1cm}
        \vspace{0.2cm}
        \begin{subfigure}[t]{0.4\textwidth}
                \centering
                \fbox{\includegraphics[height=2.5cm, width=5cm]{images/form_55_female_as_male.png}}
                \caption{}
                \label{fig:hebSection}
        \end{subfigure}
        
        \begin{subfigure}[t]{0.4\textwidth}
                \centering
                \fbox{\includegraphics[height=2.5cm, width=5cm]{images/form_51_confusing_text.png}}
                \caption{}
                \label{fig:hebSection}
        \end{subfigure}
        
        \caption{Examples of in/correct gender classification of Hebrew handwriting patch: (a)+(b) Correct male/female classification, (c)+(d) incorrect male/female classification, and (e) uncertain classification.}
        \label{fig:misclassifiedExamples}
\end{figure}

==> tables/kfold_results_fullver_tb.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\centering
\caption{Gender accuracy for form classification over 10-fold}
\label{KCrossResultsTB}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|c|c|l|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\rowcolor[HTML]{C0C0C0} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{C0C0C0}\textbf{Experiment}}                          & \textbf{Train}                                                                       & \textbf{Test}                                                                        & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}\textbf{\begin{tabular}[c]{@{}c@{}}Accuracy\\   method\end{tabular}}} & \textbf{Average} & \textbf{Std} & \textbf{fold1} & \textbf{fold2} & \textbf{fold3} & \textbf{fold4} & \textbf{fold5} & \textbf{fold6} & \textbf{fold7} & \textbf{fold8} & \textbf{fold9} & \textbf{fold10} \\ \hline
                                                                                           &                                                                                      &                                                                                      & \textbf{Majority Vote}                                                                                            & \textbf{73.02}   & 2.42         & 67.1           & 73.68          & 73.68          & 75             & 73.68          & 72.36          & 71.05          & 73.68          & 75             & 75              \\ \cline{4-16} 
                                                                                           & \multirow{-2}{*}{\textbf{Hebrew}}                                                    & \multirow{-2}{*}{\textbf{Hebrew}}                                                    & \textbf{Average Softmax}                                                                                          & 72.89            & 2.34         & 67.10          & 72.36          & 72.36          & 75.00          & 73.68          & 72.36          & 72.36          & 73.68          & 75.00          & 75              \\ \cline{2-16} 
                                                                                           &                                                                                      &                                                                                      & \textbf{Majority Vote}                                                                                            & 74.47            & 2.65         & 69.74          & 72.37          & 72.37          & 72.37          & 75.00          & 75.00          & 76.32          & 76.32          & 77.63          & 77.63           \\ \cline{4-16} 
\multirow{-4}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Language-\\ Dependent\end{tabular}}}   & \multirow{-2}{*}{\textbf{English}}                                                   & \multirow{-2}{*}{\textbf{English}}                                                   & \textbf{Average Softmax}                                                                                          & \textbf{75.26}   & 2.47         & 71.05          & 72.37          & 73.68          & 73.68          & 77.63          & 75.00          & 76.32          & 77.63          & 77.63          & 77.63           \\ \hline
                                                                                           &                                                                                      &                                                                                      & \textbf{Majority Vote}                                                                                            & 75.52            & 6.86         & 60.52          & 69.73          & 73.68          & 73.68          & 75.00          & 76.31          & 78.94          & 81.57          & 82.89          & 82.89           \\ \cline{4-16} 
                                                                                           & \multirow{-2}{*}{\textbf{Hebrew}}                                                    & \multirow{-2}{*}{\textbf{English}}                                                   & \textbf{Average Softmax}                                                                                          & \textbf{75.65}   & 7.40         & 57.89          & 69.73          & 75.00          & 75.00          & 76.31          & 77.63          & 78.94          & 80.26          & 82.89          & 82.89           \\ \cline{2-16} 
                                                                                           &                                                                                      &                                                                                      & \textbf{Majority Vote}                                                                                            & 58.29            & 5.89         & 48.68          & 50.00          & 55.26          & 56.58          & 57.89          & 59.21          & 60.53          & 64.47          & 64.47          & 65.79           \\ \cline{4-16} 
\multirow{-4}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Language-\\ Independent\end{tabular}}} & \multirow{-2}{*}{\textbf{English}}                                                   & \multirow{-2}{*}{\textbf{Hebrew}}                                                    & \textbf{Average Softmax}                                                                                          & 58.29            & 6.20         & 48.68          & 50.00          & 55.26          & 56.58          & 57.89          & 59.21          & 59.21          & 61.84          & 65.79          & 68.42           \\ \hline
                                                                                           &                                                                                      &                                                                                      & \textbf{Majority Vote}                                                                                            & \textbf{74.61}   & 2.06         & 72.37          & 72.37          & 72.37          & 73.68          & 73.68          & 75.00          & 75.00          & 76.32          & 77.63          & 77.63           \\ \cline{4-16} 
                                                                                           & \multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Hebrew+\\ English\end{tabular}}} & \multirow{-2}{*}{\textbf{Hebrew}}                                                    & \textbf{Average Softmax}                                                                                          & 73.82            & 2.36         & 68.42          & 72.37          & 72.37          & 73.68          & 73.68          & 75.00          & 75.00          & 75.00          & 76.32          & 76.32           \\ \cline{2-16} 
                                                                                           &                                                                                      &                                                                                      & \textbf{Majority Vote}                                                                                            & \textbf{79.34}   & 3.29         & 73.68          & 73.68          & 77.63          & 80.26          & 80.26          & 80.26          & 81.58          & 81.58          & 81.58          & 82.89           \\ \cline{4-16} 
                                                                                           & \multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Hebrew+\\ English\end{tabular}}} & \multirow{-2}{*}{\textbf{English}}                                                   & \textbf{Average Softmax}                                                                                          & 79.21            & 3.15         & 73.68          & 73.68          & 77.63          & 80.26          & 80.26          & 80.26          & 81.58          & 81.58          & 81.58          & 81.58           \\ \cline{2-16} 
                                                                                           &                                                                                      &                                                                                      & \textbf{Majority Vote}                                                                                            & 75.13            & 2.52         & 71.05          & 72.37          & 73.68          & 75.00          & 75.00          & 75.00          & 75.00          & 76.32          & 78.95          & 78.95           \\ \cline{4-16} 
\multirow{-6}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Mixed-\\ Languages\end{tabular}}}      & \multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Hebrew+\\ English\end{tabular}}} & \multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Hebrew+\\ English\end{tabular}}} & \textbf{Average Softmax}                                                                                          & 75.13            & 2.10         & 71.05          & 72.37          & 73.68          & 75.00          & 76.32          & 76.32          & 76.32          & 76.32          & 76.32          & 77.63           \\ \hline
\end{tabular}%
}
\end{table}

==> tables/patches_examples_res_tb.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}



%------------------------------
\begin{table}[htbp]
\caption{Predicted gender classification for examples in Fig.~\ref{fig:misclassifiedExamples}.}
\label{patches_acc_tb}
\begin{center}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{Form} & \textbf{Accuracy} & \textbf{Male Pred.} & \textbf{Female Pred.} & \multirow{2}{*}{\textbf{Prediction}} & \multirow{2}{*}{\textbf{True}}\\
\textbf{Reference} & \textbf{Method} & \textbf{Patches} & \textbf{Patches} &  & \\
\hline
\hline
\multirow{2}{*}{(a)} & Majority vote & 200 & 0 & \multirow{2}{*}{Male} & \multirow{2}{*}{Male} \\ 
& Avg. softmax & 96.24\% & 3.76\% & & \\
\hline
\multirow{2}{*}{(b)} & Majority vote & 0 & 200 & \multirow{2}{*}{Female} & \multirow{2}{*}{Female} \\ 
& Avg. softmax & 3.11\% & 96.89\% & & \\
\hline
\multirow{2}{*}{(c)} & Majority vote & 0 & 200 & \multirow{2}{*}{Female} & \multirow{2}{*}{Male} \\ 
& Avg. softmax & 5.08\% & 94.92\% & & \\
\hline
\multirow{2}{*}{(d)} & Majority vote & 170 & 30 & \multirow{2}{*}{Male} & \multirow{2}{*}{Female} \\ 
& Avg. softmax & 71.18\% & 28.82\% & & \\
\hline
\multirow{2}{*}{(e)} & Majority vote & 82 & 118 & \multirow{2}{*}{Female} & \multirow{2}{*}{Female} \\ 
& Avg. softmax & 48.15\% & 51.85\% & & \\
\hline


\end{tabular}
}
\end{center}
\end{table}
%------------------------------

